Adding Real-time Capabilities to a SML Compiler

There has been much recent interest in adopting functional and reactive programming for use in real-time system design. Moving toward a more declarative methodology for developing real-time systems purports to improve the fidelity of software. To study the benefits of functional and reactive programming for real-time systems, real-time aware functional compilers and language runtimes are required. In this paper we examine the necessary changes to a modern Standard ML compiler, MLton, to provide basic support for real-time execution. We detail our current progress in modifying MLton with a threading model that supports priorities, a chunked object model to support real-time garbage collection, and low level modification to execute on top of a real-time operating system. We present preliminary numbers and our work in progress prototype, which is able to boot ML programs compiled with MLton on x86 machines.

==> acknowledgement.tex <==
We wish to thank.. 


==> bibliography.tex <==
\bibitem{IEEEhowto:kopka}
H.~Kopka and P.~W. Daly, \emph{A Guide to \LaTeX}, 3rd~ed.\hskip 1em plus
  0.5em minus 0.4em\relax Harlow, England: Addison-Wesley, 1999.
\bibitem{MLtonThread}
M.~Fluet. (2015,Jan 15). \emph{MLtonThread}[Online].
Available:\hskip 10em
http://mlton.org/MLtonThread 



==> sec1.tex <==

\subsection{Subsection Heading Here}
Subsection text here.


\subsubsection{Subsubsection Heading Here}
Subsubsection text here.

